Efficient Human-Object-Interaction (EHOI) Detection via Interaction Label Coding and Conditional Decision

Human-Object Interaction (HOI) detection is a fundamental task in image understanding. While deep-learning-based HOI methods provide high performance in terms of mean Average Precision (mAP), they are computationally expensive and opaque in training and inference processes. An Efficient HOI (EHOI) detector is proposed in this work to strike a good balance between detection performance, inference complexity, and mathematical transparency. EHOI is a two-stage method. In the first stage, it leverages a frozen object detector to localize the objects and extract various features as intermediate outputs. In the second stage, the first-stage outputs predict the interaction type using the XGBoost classifier. Our contributions include the application of error correction codes (ECCs) to encode rare interaction cases, which reduces the model size and the complexity of the XGBoost classifier in the second stage. Additionally, we provide a mathematical formulation of the relabeling and decision-making process. Apart from the architecture, we present qualitative results to explain the functionalities of the feedforward modules. Experimental results demonstrate the advantages of ECC-coded interaction labels and the excellent balance of detection performance and complexity of the proposed EHOI method.

==> fig/DFT.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/DFT.png}
    \caption{Visualization of DFT. Red and orange dots represent the binary labels. The partition metric is the weighted sum of the left and right binary cross-entropy.}
    \label{fig: DFT}
\end{figure}

==> fig/HICO_example.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/examples.png}
    \caption{Visualization of the statistical difficulties in the HICO-DET dataset. (a) contains the unlabeled 'no\_interaction' human and object pairs; the missing labels are labeled in blue. (b)(c)(d) show the 'polysemy' in verbs. 'Wash airplane,' 'wash apple,' and 'wash carrot' share the same verb, 'wash', but the human behaves differently.}
    \label{fig: examples}
\end{figure}

==> fig/architecture.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=2.0\columnwidth]{fig/archi.png}
    \caption{The overall algorithm design of GRID. The first-stage object detector is frozen. The visual features are the filter responses from the object detector. We change the label encoding from the typical one-hot encoding to a more robust encoding.}
    \label{fig: arch}
\end{figure*}

==> fig/coding.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/coding.png}
    \caption{A toy example for four-class classification. One-vs-rest(one-hot) needs to learn a curved hyperplane for classification. Binary coding learns two straightforward decision planes and achieves a similar result by piecewise combination.}
    \label{fig: hamming}
\end{figure}

==> fig/complexity.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/bubble.png}
    \caption{Comparison between one-stage SOTAs. The x-axis is the model size in the log scale, and the y-axis is the mAP(x100) in HICO-DET under the default setting. The areas of the bubbles are proportional to the number of FLOPs.}
    \label{fig: complexity}
\end{figure}

==> fig/lose_example.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/lose_example.png}
\caption{The human representation is similar to Figure~\ref{fig: set_example}. The human query provides a probability distribution similar to that of the previous example. In contrast, the object query provides the \textit{lose} label. } \label{fig: lose_example}
\end{figure*}


==> fig/set_example.tex <==
\begin{figure*}[htbp]
\centering
\includegraphics[width=\linewidth]{fig/set_example.png}
\caption{The classifier in the human query can not find the critical representations in the umbrella region of interest. Fortunately, the object query can provide the counterparts of the prediction and make the outputs robust.} \label{fig: set_example}
\end{figure*}

